Leveraging Untrustworthy Commands for Multi-Robot Coordination in Unpredictable Environments: A Bandit Submodular Maximization Approach

We study the problem of multi-agent coordination in unpredictable and partially-observable environments with untrustworthy external commands. The commands are actions suggested to the robots, and are untrustworthy in that their performance guarantees, if any, are unknown. Such commands may be generated by human operators or machine learning algorithms and, although untrustworthy, can often increase the robots' performance in complex multi-robot tasks. We are motivated by complex multi-robot tasks such as target tracking, environmental mapping, and area monitoring. Such tasks are often modeled as submodular maximization problems due to the information overlap among the robots. We provide an algorithm, Meta Bandit Sequential Greedy (MetaBSG), which enjoys performance guarantees even when the external commands are arbitrarily bad. MetaBSG leverages a meta-algorithm to learn whether the robots should follow the commands or a recently developed submodular coordination algorithm, Bandit Sequential Greedy (BSG) [1], which has performance guarantees even in unpredictable and partially-observable environments. Particularly, MetaBSG asymptotically can achieve the better performance out of the commands and the BSG algorithm, quantifying its suboptimality against the optimal time-varying multi-robot actions in hindsight. Thus, MetaBSG can be interpreted as robustifying the untrustworthy commands. We validate our algorithm in simulated scenarios of multi-target tracking.

==> 5-fig-heuristic.tex <==
% \newcommand{\advFigColWidth}{6cm}
\begin{figure*}[t!]
    \captionsetup{font=footnotesize}
	\begin{center}
	\hspace{-9cm}
    \begin{minipage}{\columnwidth}
        \begin{tabular}{p{\introFigTitleWidth}p{\introFigColWidth}p{\introFigColWidth}p{\advFigColWidth}}%
              %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \hspace{-2mm}
        \begin{minipage}{\introFigTitleWidth}%
        \end{minipage}
        &
       \begin{minipage}{\introFigColWidth}%
              %   \vspace{-.3cm}
              \centering
              \rotatebox{0}{\sf \smaller\textbf{BSG-Meta (SG-Heuristic)}\vspace{-4cm}}
        \end{minipage}
        &            
        \begin{minipage}{\introFigColWidth}%
              %   \vspace{-.3cm}
              \centering
              \rotatebox{0}{{\sf \smaller\textbf{SG-Heuristic}}\vspace{-4cm}}
        \end{minipage}
        &
        \begin{minipage}{\advFigColWidth}%
              %   \vspace{-.3cm}
              \centering
              \rotatebox{0}{{\sf \smaller\textbf{BSG-Meta}} \textbf{\small vs.~}{\sf \smaller\textbf{BSG}} \textbf{\small vs.~}{\sf \smaller\textbf{SG-Heuristic}}\vspace{-4cm}}
        \end{minipage}
        \\
        \begin{minipage}{\introFigTitleWidth}%
              \rotatebox{90}{\textbf{2 vs.~2}\vspace{-4cm}}
        \end{minipage}
        &
        \begin{minipage}{\introFigColWidth}%
                    %   \vspace{-.3cm}
              \vspace{4mm}
              \centering%
              \includegraphics[width=.6\columnwidth]{figures/traj_2v2_meta_sg.png} \\%width=0.64\columnwidth]
              % \vspace{-2mm}
              \vspace{4mm}
              \caption*{(a) {\smaller \sf Meta}: 2 robots and 2 targets.
              }
        \end{minipage}
        &
        \begin{minipage}{\introFigColWidth}%0.6
              \vspace{5mm}
              \centering%
              \includegraphics[width=.7\columnwidth]{figures/traj_2v2_sg.png} \\ 
              % \vspace{-2mm}
              \vspace{4.8mm}
              \caption*{(c) {\smaller \sf SG\text{-}Heuristic}: 2 robots and 2 targets.
              }
        \end{minipage}
        &
        \begin{minipage}{\advFigColWidth}%
                    %   \vspace{-1mm}
              \centering%
              \hspace*{.4mm}
              \includegraphics[width=.97\columnwidth]{figures/mean_cov_2v2_sg.png} \\%0.8
              % \vspace{-2mm}
              \caption*{
              (d) {\smaller \sf Meta} vs. {\smaller \sf BSG} vs. {\smaller \sf SG\text{-}Heuristic}:
              2 robots and 2 targets.
              }
        \end{minipage}
        \\
        % \end{minipage} \\
        % \vspace{1mm}
        % \hspace{-8.9cm}
        % \begin{minipage}{\columnwidth}
        % 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \hspace{-2mm}	
        
        % \end{minipage} \\
        % \vspace{1mm}
        % \hspace{-9cm}
        % \begin{minipage}{\columnwidth}
        % 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \hspace{-2mm}	
        \begin{minipage}{0.3cm}%
              \rotatebox{90}{\textbf{2 vs.~4}\hspace{-2cm}}
        \end{minipage}
        &
        \begin{minipage}{\introFigColWidth}%
                    %   \vspace{-.3cm}
        \centering%
        \includegraphics[width=\columnwidth]{figures/traj_2v4_meta_sg.png} \\%width=0.64\columnwidth]
        % \vspace{-2mm}
        \vspace{0.6mm}
        \caption*{(e) {\smaller \sf Meta}: 2 robots and 4 targets.
        }
        \end{minipage}
        &
        \begin{minipage}{\introFigColWidth}%0.6     
        \vspace{1mm}
              \centering%
        \includegraphics[width=\columnwidth]{figures/traj_2v4_sg.png} \\ 
        % \vspace{-2mm}
        \vspace{2.5mm}
        \caption*{(g) {\smaller \sf SG\text{-}Heuristic}: 2 robots and 4 targets.
        }
        \end{minipage}
        &
        \begin{minipage}{\advFigColWidth}%
                    %   \vspace{-.3cm}
        \centering%
        \includegraphics[width=\columnwidth]{figures/mean_cov_2v4_sg.png} \\%0.8
         \vspace{-3mm}
        %\vspace{0.2mm}
        \hspace{-1mm}
        \caption*{(h) {\smaller \sf Meta} vs. {\smaller \sf BSG} vs. {\smaller \sf SG\text{-}Heuristic}:
        2 robots and 4 targets.
        }
        \end{minipage}
        \end{tabular}
\end{minipage} 
% 	\vspace{-1mm}
	\caption{\textbf{Multi-Robot Target Tracking with SG-Heuristic Advice: $2$ Robots Pursuing $2$ or $4$ Targets.} 
	The robots select actions per {\smaller \sf Meta}, {\smaller \sf BSG}, or per the greedy heuristic {\smaller \sf SG\text{-}Heuristic}, re-selecting actions with frequency $20$Hz. Across the two algorithm cases, the targets traverse the same predefined trajectories, which are non-adaptive to the robots' motion.(a),(e): The robots use {\smaller \sf Meta} against $2$ and $4$ targets, respectively; (b),(f): The robots use {\smaller \sf BSG} against $2$ and $4$ targets, respectively; (c), (g): The robots use {\smaller \sf SG\text{-}Heuristic} against $2$ and $4$ targets, respectively. (d),(h): Comparison of {\smaller \sf Meta}'s, {\smaller \sf BSG}'s and {\smaller \sf SG\text{-}Heuristic}'s  \mbox{average effectiveness over $50$ Monte-Carlo trials.}
	}\label{fig:heuristic}
	\vspace{-9mm}
	\end{center}
\end{figure*}


==> 5-fig-scenario.tex <==
\begin{figure}[b!]
    \captionsetup{font=footnotesize}
    \centering
    \includegraphics[width=.\columnwidth]{figures/traj_2v4_BSG_demo.png}\\
    \caption{\textbf{Target Tracking Instance of Two Robots Tracking Four Targets.} Two robots with a limited 
    sensing range and a limited angle of 
    view collaboratively track the locations of four targets moving on a plane. Each robot obtains range and bearing measurements of a target only when the target is inside the robot's field of view.
    The sensors' noise is assumed zero-mean Gaussian, with increasing variance the further away the target is from the robot.
    Target outside the field of view of a robot are unobservable.
    The targets' motion model is unknown to the robots.
    The robots coordinate based only on the past observations. 
    }\label{fig:partial-sim}
\end{figure}
